STLGT: A Scalable Trace-Based Linear Graph Transformer for Tail Latency Prediction in Microservices

Accurate end-to-end tail-latency forecasting is critical for proactive SLO management in microservice systems. However, modeling long-range dependency propagation and non-stationary, bursty workloads while maintaining inference efficiency at scale remains challenging. We present STLGT (Scalable Trace-based Linear Graph Transformer), a per-API predictor that encodes traces as span graphs for multi-step p95 tail-latency forecasting. STLGT uses a structure-aware linear graph Transformer to propagate cross-service dependencies with inference time linear in span graph size, and a decoupled temporal module to capture workload dynamics. Across a personalized education microservice application, DeathStarBench, and Alibaba traces, STLGT improves forecasting accuracy over PERT-GNN by 8.5% MAPE on average and achieves up to 12x faster CPU inference at N=32, matching the maximum span graph size after preprocessing the Alibaba traces. Ablation studies further demonstrate the effectiveness of each component, especially under bursty traffic.

==> sections/method/4-1-definition.tex <==
As mentioned in Sec.~\ref{sec:introduction}, we study tail-latency prediction for a target Remote Procedure Call (RPC) endpoint $\mathcal{A}$ in a microservice application. We represent inter-service invocations as a \emph{Microservice Call Graph (MCG)}. We discretize time into windows of length $\Delta$ and use $t$ to index windows. Given observations up to window $t$, we predict the tail latency of $\mathcal{A}$ over the next $H$ windows.

We abstract the microservice cluster as a directed graph:

\begin{equation}
  \mathcal{G} = (\mathcal{V}, \mathcal{E})
\end{equation}
where $\mathcal{V}$ denotes the set of microservices with $|\mathcal{V}| = M$, and $\mathcal{E}$ represents directed invocation relations $s_{\text{in}} \!\to s_{\text{out}}$ between services. In typical deployments, the call graph is sparse, i.e., $|\mathcal{E}| \ll M^{2}$.

For a given RPC $\mathcal{A}$, we further construct its \textbf{Span Graph}:

\begin{equation}
  \mathcal{G}^{\mathcal{A}} = (\mathcal{V}^{\mathcal{A}}, \mathcal{E}^{\mathcal{A}})
\end{equation}
where $\mathcal{V}^{\mathcal{A}}$ is the set of execution-stage nodes induced from traces, and $\mathcal{E}^{\mathcal{A}}$ encodes trace-derived dependencies between stages. We define a surjective mapping $\pi:\mathcal{V}^{\mathcal{A}}\rightarrow\mathcal{V}$ that maps each stage node to its corresponding microservice.
Let $\mathcal{T}^{\mathcal{A}}_{t}$ be the set of traces of $\mathcal{A}$ collected in window $t$. Each trace contains a set of spans, and spans are the basic invocation records used to construct stage-level features. Meanwhile, each microservice $s\in\mathcal{V}$ at time step $t$ is characterized by a service-level resource/runtime metric vector of dimension $d_{s}$. Accordingly, we consider two types of runtime observations.

\paragraph{Service-level metrics}
\begin{equation}
  \mathcal{M}^{(s)}_{t}=\{ \mathbf{m}^{s}_{t}\in\mathbb{R}^{d_{s}} \mid s\in\mathcal{V} \}
\end{equation}

\paragraph{Trace aggregation and node features}
Raw traces must be aggregated into window-aligned learning signals. We extract a trace-common vector and per-stage span-specific vectors by
\begin{equation}
  \mathbf{c}^{\mathcal{A}}_{t}=\phi_{\text{common}}\big(\mathcal{T}^{\mathcal{A}}_{t}\big)\in\mathbb{R}^{d_{c}},\qquad
  \mathbf{u}^{\mathcal{A}}_{t,i}=\phi_{\text{span}}\big(\mathcal{T}^{\mathcal{A}}_{t},\ v^{\mathcal{A}}_{i}\big)\in\mathbb{R}^{d_{u}},
\end{equation}
where $\phi_{\text{common}}(\cdot)$ summarizes API-level workload/performance signals (trace-common), and $\phi_{\text{span}}(\cdot)$ summarizes fine-grained timing structure for each stage node (span-specific).
We then construct the stage-node feature for $v^{\mathcal{A}}_{i}$ in window $t$ as
\begin{equation}
  \mathbf{x}^{\mathcal{A}}_{t,i}
  =
  \Big[
    \mathbf{m}^{\pi(v^{\mathcal{A}}_{i})}_{t}\ \Vert\ \mathbf{u}^{\mathcal{A}}_{t,i}
  \Big],
\end{equation}
and stack all stage-node features into a node-feature matrix $\mathbf{X}^{\mathcal{A}}_{t}\in\mathbb{R}^{|\mathcal{V}^{\mathcal{A}}|\times d_{in}}$ for subsequent encoding. The trace-common vector $\mathbf{c}^{\mathcal{A}}_{t}$ is used as a window-level context in the trace-aware readout (Sec.~\ref{sec:latency-predictor}).

In production microservices, the same API endpoint may traverse different service chains at runtime due to conditional control flow (e.g., if--else guards, feature flags, fallbacks, and retries). While one could build a unified model that pools traces from multiple call paths and learns to handle such path variability, this is an implementation choice that is separate from the core modeling components studied in this paper. For clarity, we treat each distinct call path as a separate RPC $\mathcal{A}$. Consequently, the structure of $\mathcal{G}^{\mathcal{A}}$ (equivalently, its adjacency matrix) can be viewed as a \textbf{time-invariant sparse matrix}, and the temporal dynamics are primarily captured by the evolution of node features $\mathbf{X}^{\mathcal{A}}_{t}$.

Therefore, given the history length $L$ and the prediction horizon $H$, our task can be formulated as a supervised graph-temporal regression problem:
\begin{equation}
  \hat{\mathbf{y}}^{\mathcal{A}}_{t+1:t+H}
  = f_{\theta}\Big(\mathcal{G}^{\mathcal{A}},\ \mathbf{X}^{\mathcal{A}}_{t-L+1:t},\ \mathbf{c}^{\mathcal{A}}_{t-L+1:t}\Big)\in\mathbb{R}^{H}
  \label{eq:prediction}
\end{equation}

